Planet Masses, Radii, and Orbits from NASA's K2 Mission

We report the masses, sizes, and orbital properties of 86 planets orbiting 55 stars observed by NASA's K2 Mission with follow-up Doppler measurements by the HIRES spectrometer at the W. M. Keck Observatory and the Automated Planet Finder at Lick Observatory. Eighty-one of the planets were discovered from their transits in the K2 photometry, while five were found based on subsequent Doppler measurements of transiting planet host stars. The sizes of the transiting planets range from Earth-size to larger than Jupiter (1-3 REarth is typical), while the orbital periods range from less than a day to a few months. For 32 of the planets, the Doppler signal was detected with significance greater than 5-sigma (51 were detected with >3-sigma significance). An important characteristic of this catalog is the use of uniform analysis procedures to determine stellar and planetary properties. This includes the transit search and fitting procedures applied to the K2 photometry, the Doppler fitting techniques applied to the radial velocities, and the spectral modeling to determine bulk stellar parameters. Such a uniform treatment will make the catalog useful for statistical studies of the masses, densities, and system architectures of exoplanetary systems. This work also serves as a data release for all previously unpublished RVs and associated stellar activity indicators obtained by our team for these systems, along with derived stellar and planet parameters.

==> epic202089657.tex <==
\subsection{EPIC 202089657} % 202089657 - jgfh

% http://simbad.harvard.edu/simbad/sim-id?Ident=EPIC202089657&NbIdent=1&Radius=2&Radius.unit=arcmin&submit=submit+id 

Notes: In catalog of \cite{Vanderburg2016-catalog}.
\red{Add Crossfield+2016}

\jgfhSTNAME
is a \red{SPECTRAL-TYPE} with \red{NN} transiting planets that have sizes \red{[SIZES]} and orbital periods \red{[ORBITAL PERIODS]}.
\red{Comment on catalogs in which the planet was found.}
See Tables \ref{tb:star_pars}  and \ref{tb:star_props} for stellar properties and Table \ref{tb:planet_props} for precise planet parameters.
\red{ADD Comments from literature search about discovery (other papers/catalogs), validation, differences in stellar parameters, etc.}  Our fit of the EVEREST light curve of the K2 photometry for \jgfhSTNAME is shown in Fig.\ \ref{fig:lc_epic202089657}.

\begin{figure*}
\epsscale{1.0}
\plotone{202089657-fits-final.png}
\caption{Time series (top) and phase-folded (bottom) light curve for the planet orbiting \jgfhSTNAME.  Plot formatting is the same as in Fig.\ \ref{fig:lc_epic220709978}.}
\label{fig:lc_epic202089657}
\end{figure*}

We acquired \red{NN} %\xxxxNOBSHIRES 
RVs of \red{[STARNAME}] with HIRES, typically with an exposure meter setting of \red{XXX}.  
\red{Comment on chromospheric activity, if active.}  
We modeled the system as \red{[fill in details about RV model (Nplanets, eccentricity, priors)]}.  The results of this analysis are listed in Table 
\red{TABLE REF} % \ref{tab:epicxxxxxxxxx}
and the best-fit model is shown in Fig.\ 
\red{[FIG REF]}. %\ref{}.
\red{[PLANET NAME]} is a \red{[DESCRIPTION OF THE PLANET]}.

\red{COMMENT on model fit (good/bad), jitter, jitter of other instruments.}

\red{COMMENT on model comparison (eccentricity, dvdt).}

\red{COMMENT on (dis-)agreement with other studies.}

\red{COMMENT on prospects for future measurements.}

\red{ADD paragraph about validation, if needed.}

% note: 4 nights (18 RVs), triple shots -- note that system is not validated
% in Crossfield; in Mayo - "VESPA failed to find a FPP."

\red{Sarah's notes: see latex comments in this section-- should be drop this star? In the meantime, I've adopted a circular model for simplicity.}

\import{}{epic202089657_circ_priors+params.tex}

\begin{figure}
\epsscale{1.0}
\plotone{keyproj_epic202089657_circ_rv_multipanel.pdf}
\caption{RVs and Keplerian model for \jgfhSTNAME.  Symbols, lines, and annotations are similar to those in Fig.\ \ref{fig:rvs_epic220709978}.}
\label{fig:rvs_202089657}
\end{figure}



==> epic247418783.tex <==
\subsection{EPIC 247418783} % EPIC 247418783 - ihid
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% http://simbad.harvard.edu/simbad/sim-id?Ident=EPIC247418783&NbIdent=1&Radius=2&Radius.unit=arcmin&submit=submit+id 

%Don't use this file, use K2-291 below!

\ihidSTNAME is a solar-type star from Campaign 13 that has one transiting planet with a radius of 1.7 \rearth and an orbital period of 2.2 days. 
The host star has elevated activity with \lrphk = \ihidRPHK dex.
\ihidPNAMEone was recent characterized by \citet{Kosiarek2019b} and we adopt the parameters of their analysis of HIRES and HARPS-N RVs using a GP model.  
See Tables \ref{tb:star_pars}  and \ref{tb:star_props} for stellar properties and Table \ref{tb:planet_props} for precise planet parameters.

\red{Change star name to K2-291}
\red{Add planet parameters from Kosiarek2019}

==> generic.tex <==
\subsection{Generic New Planet}

% link to Simbad
% note with EPIC name and latex code

\red{STARNAME} % \xxxxSTNAME
is a \red{SPECTRAL-TYPE} with \red{NN} transiting planets that have sizes \red{[SIZES]} and orbital periods \red{[ORBITAL PERIODS]}.
\red{Comment on catalogs in which the planet was found.}
See Tables \ref{tb:star_pars}  and \ref{tb:star_props} for stellar properties and Table \ref{tb:planet_props} for precise planet parameters.
\red{ADD Comments from literature search about discovery (other papers/catalogs), validation, differences in stellar parameters, etc.}  Our fit of the EVEREST light curve of the K2 photometry for \red{STARNAME} %\xxxxSTNAME 
is shown in Fig.\ \ref{fig:lc_epicxxxxxxxxx}.

\begin{figure*}
\epsscale{1.0}
\plotone{xxxxxxxxx-fits-final.png}
\caption{Time series (top) and phase-folded (bottom) light curve for the planet orbiting \red{STARNAME}% \xxxxSTNAME
.  Plot formatting is the same as in Fig.\ \ref{fig:lc_epic201437844}.}
\label{fig:lc_epicxxxxxxxxx}
\end{figure*}

We acquired \red{NN} %\xxxxNOBSHIRES 
RVs of \red{[STARNAME}] with HIRES, typically with an exposure meter setting of \red{XXX}.  
\red{Comment on chromospheric activity, if active.}  
We modeled the system as \red{[fill in details about RV model (Nplanets, eccentricity, priors)]}.  The results of this analysis are listed in Table 
\red{TABLE REF} % \ref{tab:epicxxxxxxxxx}
and the best-fit model is shown in Fig.\ 
\red{[FIG REF]}. %\ref{}.
\red{[PLANET NAME]} is a \red{[DESCRIPTION OF THE PLANET]}.

\red{COMMENT on model fit (good/bad), jitter, jitter of other instruments.}

\red{COMMENT on model comparison (eccentricity, dvdt).}

\red{COMMENT on (dis-)agreement with other studies.}

\red{COMMENT on prospects for future measurements.}

\red{ADD paragraph about validation, if needed.}


% Plot formatting is the same as in Fig.~\ref{fig:lc_epic220709978}.
% Symbols, lines, and annotations are similar to those in Fig.\ \ref{fig:rvs_epic220709978}.
% Lines and annotations are similar to those in Fig.\ \ref{fig:rvs_epic220709978_resid}.

%\import{tables/xxx_circ_priors+params.tex}{}

\begin{figure}
\epsscale{1.0}
%\plotone{xxx_circ_rv_multipanel.pdf}
\caption{RVs and Keplerian model for \red{ADD NAME}. % \xxxxSTNAME
Symbols, lines, and annotations are similar to those in Fig.\ \ref{fig:rvs_epic220709978}.}
\label{fig:rvs_XXX}
\end{figure}


%\begin{figure}
%\epsscale{1.0}
%\plotone{2DKLS_epicxxxxxxxxx_circ_per_2_paperversion.png}
%\caption{Periodogram search of the RVs for \xxxxSTNAME showing no evidence for a second planet.  Lines and annotations are similar to those in Fig.\ \ref{fig:rvs_epic220709978_resid}.}
%\label{fig:rvs_epicxxxxxxxxx_resid}
%\end{figure}


==> table_st_pars.tex <==
\ddigSTNAME & \ddigSTNAMEKTWO & \ddigEPICID & \ddigCAMPAIGN & \ddigRA & \ddigDEC & \ddigVMAG & \ddigNOBSHIRES & \ddigNOBSAPF & \ddigNOBSOTHER \\
\bdiaSTNAME & \bdiaSTNAMEKTWO & \bdiaEPICID & \bdiaCAMPAIGN & \bdiaRA & \bdiaDEC & \bdiaVMAG & \bdiaNOBSHIRES & \bdiaNOBSAPF & \bdiaNOBSOTHER \\
\hieeSTNAME & \hieeSTNAMEKTWO & \hieeEPICID & \hieeCAMPAIGN & \hieeRA & \hieeDEC & \hieeVMAG & \hieeNOBSHIRES & \hieeNOBSAPF & \hieeNOBSOTHER \\
\hbagSTNAME & \hbagSTNAMEKTWO & \hbagEPICID & \hbagCAMPAIGN & \hbagRA & \hbagDEC & \hbagVMAG & \hbagNOBSHIRES & \hbagNOBSAPF & \hbagNOBSOTHER \\
\jjhiSTNAME & \jjhiSTNAMEKTWO & \jjhiEPICID & \jjhiCAMPAIGN & \jjhiRA & \jjhiDEC & \jjhiVMAG & \jjhiNOBSHIRES & \jjhiNOBSAPF & \jjhiNOBSOTHER \\
\ihidSTNAME & \ihidSTNAMEKTWO & \ihidEPICID & \ihidCAMPAIGN & \ihidRA & \ihidDEC & \ihidVMAG & \ihidNOBSHIRES & \ihidNOBSAPF & \ihidNOBSOTHER \\
\fcabSTNAME & \fcabSTNAMEKTWO & \fcabEPICID & \fcabCAMPAIGN & \fcabRA & \fcabDEC & \fcabVMAG & \fcabNOBSHIRES & \fcabNOBSAPF & \fcabNOBSOTHER \\
\eidfSTNAME & \eidfSTNAMEKTWO & \eidfEPICID & \eidfCAMPAIGN & \eidfRA & \eidfDEC & \eidfVMAG & \eidfNOBSHIRES & \eidfNOBSAPF & \eidfNOBSOTHER \\
\hehhSTNAME & \hehhSTNAMEKTWO & \hehhEPICID & \hehhCAMPAIGN & \hehhRA & \hehhDEC & \hehhVMAG & \hehhNOBSHIRES & \hehhNOBSAPF & \hehhNOBSOTHER \\
\jifiSTNAME & \jifiSTNAMEKTWO & \jifiEPICID & \jifiCAMPAIGN & \jifiRA & \jifiDEC & \jifiVMAG & \jifiNOBSHIRES & \jifiNOBSAPF & \jifiNOBSOTHER \\
\iahiSTNAME & \iahiSTNAMEKTWO & \iahiEPICID & \iahiCAMPAIGN & \iahiRA & \iahiDEC & \iahiVMAG & \iahiNOBSHIRES & \iahiNOBSAPF & \iahiNOBSOTHER \\
\aiggSTNAME & \aiggSTNAMEKTWO & \aiggEPICID & \aiggCAMPAIGN & \aiggRA & \aiggDEC & \aiggVMAG & \aiggNOBSHIRES & \aiggNOBSAPF & \aiggNOBSOTHER \\
\jgjjSTNAME & \jgjjSTNAMEKTWO & \jgjjEPICID & \jgjjCAMPAIGN & \jgjjRA & \jgjjDEC & \jgjjVMAG & \jgjjNOBSHIRES & \jgjjNOBSAPF & \jgjjNOBSOTHER \\
\hhedSTNAME & \hhedSTNAMEKTWO & \hhedEPICID & \hhedCAMPAIGN & \hhedRA & \hhedDEC & \hhedVMAG & \hhedNOBSHIRES & \hhedNOBSAPF & \hhedNOBSOTHER \\
\befbSTNAME & \befbSTNAMEKTWO & \befbEPICID & \befbCAMPAIGN & \befbRA & \befbDEC & \befbVMAG & \befbNOBSHIRES & \befbNOBSAPF & \befbNOBSOTHER \\
% \jgfhSTNAME & \jgfhSTNAMEKTWO & \jgfhEPICID & \jgfhCAMPAIGN & \jgfhRA & \jgfhDEC & \jgfhVMAG & \jgfhNOBSHIRES & \jgfhNOBSAPF & \jgfhNOBSOTHER \\
\eaccSTNAME & \eaccSTNAMEKTWO & \eaccEPICID & \eaccCAMPAIGN & \eaccRA & \eaccDEC & \eaccVMAG & \eaccNOBSHIRES & \eaccNOBSAPF & \eaccNOBSOTHER \\
\dcijSTNAME & \dcijSTNAMEKTWO & \dcijEPICID & \dcijCAMPAIGN & \dcijRA & \dcijDEC & \dcijVMAG & \dcijNOBSHIRES & \dcijNOBSAPF & \dcijNOBSOTHER \\
\bejgSTNAME & \bejgSTNAMEKTWO & \bejgEPICID & \bejgCAMPAIGN & \bejgRA & \bejgDEC & \bejgVMAG & \bejgNOBSHIRES & \bejgNOBSAPF & \bejgNOBSOTHER \\
\bajiSTNAME & \bajiSTNAMEKTWO & \bajiEPICID & \bajiCAMPAIGN & \bajiRA & \bajiDEC & \bajiVMAG & \bajiNOBSHIRES & \bajiNOBSAPF & \bajiNOBSOTHER \\
\bcgdSTNAME & \bcgdSTNAMEKTWO & \bcgdEPICID & \bcgdCAMPAIGN & \bcgdRA & \bcgdDEC & \bcgdVMAG & \bcgdNOBSHIRES & \bcgdNOBSAPF & \bcgdNOBSOTHER \\
\fffdSTNAME & \fffdSTNAMEKTWO & \fffdEPICID & \fffdCAMPAIGN & \fffdRA & \fffdDEC & \fffdVMAG & \fffdNOBSHIRES & \fffdNOBSAPF & \fffdNOBSOTHER \\
\ecdcSTNAME & \ecdcSTNAMEKTWO & \ecdcEPICID & \ecdcCAMPAIGN & \ecdcRA & \ecdcDEC & \ecdcVMAG & \ecdcNOBSHIRES & \ecdcNOBSAPF & \ecdcNOBSOTHER \\
\dcbjSTNAME & \dcbjSTNAMEKTWO & \dcbjEPICID & \dcbjCAMPAIGN & \dcbjRA & \dcbjDEC & \dcbjVMAG & \dcbjNOBSHIRES & \dcbjNOBSAPF & \dcbjNOBSOTHER \\
\ddeiSTNAME & \ddeiSTNAMEKTWO & \ddeiEPICID & \ddeiCAMPAIGN & \ddeiRA & \ddeiDEC & \ddeiVMAG & \ddeiNOBSHIRES & \ddeiNOBSAPF & \ddeiNOBSOTHER \\
\fdijSTNAME & \fdijSTNAMEKTWO & \fdijEPICID & \fdijCAMPAIGN & \fdijRA & \fdijDEC & \fdijVMAG & \fdijNOBSHIRES & \fdijNOBSAPF & \fdijNOBSOTHER \\
\gafeSTNAME & \gafeSTNAMEKTWO & \gafeEPICID & \gafeCAMPAIGN & \gafeRA & \gafeDEC & \gafeVMAG & \gafeNOBSHIRES & \gafeNOBSAPF & \gafeNOBSOTHER \\
\bhiiSTNAME & \bhiiSTNAMEKTWO & \bhiiEPICID & \bhiiCAMPAIGN & \bhiiRA & \bhiiDEC & \bhiiVMAG & \bhiiNOBSHIRES & \bhiiNOBSAPF & \bhiiNOBSOTHER \\
\bbggSTNAME & \bbggSTNAMEKTWO & \bbggEPICID & \bbggCAMPAIGN & \bbggRA & \bbggDEC & \bbggVMAG & \bbggNOBSHIRES & \bbggNOBSAPF & \bbggNOBSOTHER \\
\dbfaSTNAME & \dbfaSTNAMEKTWO & \dbfaEPICID & \dbfaCAMPAIGN & \dbfaRA & \dbfaDEC & \dbfaVMAG & \dbfaNOBSHIRES & \dbfaNOBSAPF & \dbfaNOBSOTHER \\
\ccdhSTNAME & \ccdhSTNAMEKTWO & \ccdhEPICID & \ccdhCAMPAIGN & \ccdhRA & \ccdhDEC & \ccdhVMAG & \ccdhNOBSHIRES & \ccdhNOBSAPF & \ccdhNOBSOTHER \\
\eicdSTNAME & \eicdSTNAMEKTWO & \eicdEPICID & \eicdCAMPAIGN & \eicdRA & \eicdDEC & \eicdVMAG & \eicdNOBSHIRES & \eicdNOBSAPF & \eicdNOBSOTHER \\
\bggeSTNAME & \bggeSTNAMEKTWO & \bggeEPICID & \bggeCAMPAIGN & \bggeRA & \bggeDEC & \bggeVMAG & \bggeNOBSHIRES & \bggeNOBSAPF & \bggeNOBSOTHER \\
\hagfSTNAME & \hagfSTNAMEKTWO & \hagfEPICID & \hagfCAMPAIGN & \hagfRA & \hagfDEC & \hagfVMAG & \hagfNOBSHIRES & \hagfNOBSAPF & \hagfNOBSOTHER \\
\gcidSTNAME & \gcidSTNAMEKTWO & \gcidEPICID & \gcidCAMPAIGN & \gcidRA & \gcidDEC & \gcidVMAG & \gcidNOBSHIRES & \gcidNOBSAPF & \gcidNOBSOTHER \\
\jfjgSTNAME & \jfjgSTNAMEKTWO & \jfjgEPICID & \jfjgCAMPAIGN & \jfjgRA & \jfjgDEC & \jfjgVMAG & \jfjgNOBSHIRES & \jfjgNOBSAPF & \jfjgNOBSOTHER \\
\baeiSTNAME & \baeiSTNAMEKTWO & \baeiEPICID & \baeiCAMPAIGN & \baeiRA & \baeiDEC & \baeiVMAG & \baeiNOBSHIRES & \baeiNOBSAPF & \baeiNOBSOTHER \\
\bjieSTNAME & \bjieSTNAMEKTWO & \bjieEPICID & \bjieCAMPAIGN & \bjieRA & \bjieDEC & \bjieVMAG & \bjieNOBSHIRES & \bjieNOBSAPF & \bjieNOBSOTHER \\
\gghbSTNAME & \gghbSTNAMEKTWO & \gghbEPICID & \gghbCAMPAIGN & \gghbRA & \gghbDEC & \gghbVMAG & \gghbNOBSHIRES & \gghbNOBSAPF & \gghbNOBSOTHER \\
\ggacSTNAME & \ggacSTNAMEKTWO & \ggacEPICID & \ggacCAMPAIGN & \ggacRA & \ggacDEC & \ggacVMAG & \ggacNOBSHIRES & \ggacNOBSAPF & \ggacNOBSOTHER \\
\egijSTNAME & \egijSTNAMEKTWO & \egijEPICID & \egijCAMPAIGN & \egijRA & \egijDEC & \egijVMAG & \egijNOBSHIRES & \egijNOBSAPF & \egijNOBSOTHER \\
\hadfSTNAME & \hadfSTNAMEKTWO & \hadfEPICID & \hadfCAMPAIGN & \hadfRA & \hadfDEC & \hadfVMAG & \hadfNOBSHIRES & \hadfNOBSAPF & \hadfNOBSOTHER \\
\hidfSTNAME & \hidfSTNAMEKTWO & \hidfEPICID & \hidfCAMPAIGN & \hidfRA & \hidfDEC & \hidfVMAG & \hidfNOBSHIRES & \hidfNOBSAPF & \hidfNOBSOTHER \\
\bebbSTNAME & \bebbSTNAMEKTWO & \bebbEPICID & \bebbCAMPAIGN & \bebbRA & \bebbDEC & \bebbVMAG & \bebbNOBSHIRES & \bebbNOBSAPF & \bebbNOBSOTHER \\
\ecdiSTNAME & \ecdiSTNAMEKTWO & \ecdiEPICID & \ecdiCAMPAIGN & \ecdiRA & \ecdiDEC & \ecdiVMAG & \ecdiNOBSHIRES & \ecdiNOBSAPF & \ecdiNOBSOTHER \\
\gedgSTNAME & \gedgSTNAMEKTWO & \gedgEPICID & \gedgCAMPAIGN & \gedgRA & \gedgDEC & \gedgVMAG & \gedgNOBSHIRES & \gedgNOBSAPF & \gedgNOBSOTHER \\
\jgbhSTNAME & \jgbhSTNAMEKTWO & \jgbhEPICID & \jgbhCAMPAIGN & \jgbhRA & \jgbhDEC & \jgbhVMAG & \jgbhNOBSHIRES & \jgbhNOBSAPF & \jgbhNOBSOTHER \\
\ghijSTNAME & \ghijSTNAMEKTWO & \ghijEPICID & \ghijCAMPAIGN & \ghijRA & \ghijDEC & \ghijVMAG & \ghijNOBSHIRES & \ghijNOBSAPF & \ghijNOBSOTHER \\
\fdecSTNAME & \fdecSTNAMEKTWO & \fdecEPICID & \fdecCAMPAIGN & \fdecRA & \fdecDEC & \fdecVMAG & \fdecNOBSHIRES & \fdecNOBSAPF & \fdecNOBSOTHER \\
\deffSTNAME & \deffSTNAMEKTWO & \deffEPICID & \deffCAMPAIGN & \deffRA & \deffDEC & \deffVMAG & \deffNOBSHIRES & \deffNOBSAPF & \deffNOBSOTHER \\
\hbdaSTNAME & \hbdaSTNAMEKTWO & \hbdaEPICID & \hbdaCAMPAIGN & \hbdaRA & \hbdaDEC & \hbdaVMAG & \hbdaNOBSHIRES & \hbdaNOBSAPF & \hbdaNOBSOTHER \\
\eiadSTNAME & \eiadSTNAMEKTWO & \eiadEPICID & \eiadCAMPAIGN & \eiadRA & \eiadDEC & \eiadVMAG & \eiadNOBSHIRES & \eiadNOBSAPF & \eiadNOBSOTHER \\
\ifgjSTNAME & \ifgjSTNAMEKTWO & \ifgjEPICID & \ifgjCAMPAIGN & \ifgjRA & \ifgjDEC & \ifgjVMAG & \ifgjNOBSHIRES & \ifgjNOBSAPF & \ifgjNOBSOTHER \\
\cffcSTNAME & \cffcSTNAMEKTWO & \cffcEPICID & \cffcCAMPAIGN & \cffcRA & \cffcDEC & \cffcVMAG & \cffcNOBSHIRES & \cffcNOBSAPF & \cffcNOBSOTHER \\
\egbeSTNAME & \egbeSTNAMEKTWO & \egbeEPICID & \egbeCAMPAIGN & \egbeRA & \egbeDEC & \egbeVMAG & \egbeNOBSHIRES & \egbeNOBSAPF & \egbeNOBSOTHER \\
\fdfaSTNAME & \fdfaSTNAMEKTWO & \fdfaEPICID & \fdfaCAMPAIGN & \fdfaRA & \fdfaDEC & \fdfaVMAG & \fdfaNOBSHIRES & \fdfaNOBSAPF & \fdfaNOBSOTHER \\

